Grasp selection analysis for two-step manipulation tasks

Manipulation tasks are sequential in nature. Grasp selection approaches that take into account the con- straints at each task step are critical, since they allow to both (1) Identify grasps that likely require simple arm motions through the whole task and (2) To discard grasps that, although feasible to achieve at earlier steps, might not be executable at later stages due to goal task constraints. In this paper, we study how to use our previously proposed manipulation metric for tasks in which 2 steps are required (pick-and-place and pouring tasks). Even for such simple tasks, it was not clear how to use the results of applying our metric (or any metric for that matter) to rank all the candidate grasps: Should only the start state be considered, or only the goal, or a combination of both? In order to find an answer, we evaluated the (best) grasps selected by our metric under each of these 3 considerations. Our main conclusion was that for tasks in which the goal state is more constrained (pick-and-place), using a combination of the metric measured at the start and goal states renders better performance when compared with choosing any other candidate grasp, whereas in tasks in which the goal constraints are less rigidly defined, the metric measured at the start state should be mainly considered. We present quantitative results in simulation and validate our approach's practicality with experimental results in our physical robot manipulator, Crichton.

==> experimentImages.tex <==
%-------------------------
% PaP plushie
%-------------------------
\begin{figure}[t]
\centering
\begin{tikzpicture}[framed,background rectangle/.style={thick,draw=black,fill=bgcolor,rounded corners=1em}]
\node[]{\includegraphics[width=0.45\textwidth]{./figures/pap_mike_3_scenarios.jpg}};
%\draw[line width=0.75mm, white] (-4,0) -- (4,0);
\node[text=blue,xshift=0cm,yshift=4.25cm,fill=white,fill opacity=0.5]{~~~~~~~~~~~~~Put plushie inside the box~~~~~~~~~~~~~~~};
\node[text=blue,xshift=-2.0cm,yshift=1.75cm]{Start};
\node[text=blue,xshift=2.0cm,yshift=1.75cm]{Goal};
\node[text=blue,xshift=0cm,yshift=1.25cm,fill=white,fill opacity=0.5]{~~~~~~~~~~~~~Put plushie inside the  box~~~~~~~~~~~~~~};
\node[text=blue,xshift=-2.0cm,yshift=-1.25cm]{Start};
\node[text=blue,xshift=2.0cm,yshift=-1.25cm]{Goal};
\node[text=blue,xshift=0cm,yshift=-1.75cm,fill=white,fill opacity=0.5]{~~~~~Put plushie somewhere else on the table ~~~~~~};
\node[text=blue,xshift=-2.0cm,yshift=-4.25cm]{Start};
\node[text=blue,xshift=2.0cm,yshift=-4.25cm]{Goal};
\end{tikzpicture}
\caption{Pick-and-place tasks: According to the task, the grasp selected varies}
\label{fig:pap_plushie}
\vspace{-2.0em}
\end{figure}

%-------------------------
% PaP cheezit
%-------------------------
\begin{figure}[h]
\centering
\begin{tikzpicture}[framed,background rectangle/.style={thick,draw=black,fill=bgcolor,rounded corners=1em}]
\node[]{\includegraphics[width=0.45\textwidth]{./figures/pap_cheezit_3_scenarios.jpg}};
%\draw[line width=0.75mm, white] (-4,0) -- (4,0);
\node[text=blue,xshift=0cm,yshift=4.25cm,fill=white,fill opacity=0.5]{~~~~~~~~~~~~~Put Cheezit inside the box~~~~~~~~~~~~~~~};
\node[text=blue,xshift=-2.0cm,yshift=1.75cm]{Start};
\node[text=blue,xshift=2.0cm,yshift=1.75cm]{Goal};
\node[text=blue,xshift=0cm,yshift=1.25cm,fill=white,fill opacity=0.5]{~~~~~~~~~~~~~Put Cheezit inside the  box~~~~~~~~~~~~~~};
\node[text=blue,xshift=-2.0cm,yshift=-1.25cm]{Start};
\node[text=blue,xshift=2.0cm,yshift=-1.25cm]{Goal};
\node[text=blue,xshift=0cm,yshift=-1.75cm,fill=white,fill opacity=0.5]{~~~~~Put Cheezit somewhere else on the table ~~~~~~};
\node[text=blue,xshift=-2.0cm,yshift=-4.25cm]{Start};
\node[text=blue,xshift=2.0cm,yshift=-4.25cm]{Goal};
\end{tikzpicture}
\caption{Pick-and-place tasks: According to the task, the grasp selected varies}
\label{fig:pap_plushie}
\vspace{-2.0em}
\end{figure}

%-------------------------
% PaP cheezit
%-------------------------
\begin{figure}[h]
\centering
\begin{tikzpicture}[framed,background rectangle/.style={thick,draw=black,fill=bgcolor,rounded corners=1em}]
\node[]{\includegraphics[width=0.45\textwidth]{./figures/pouring_3_objects_bowl.jpg}};
%\draw[line width=0.75mm, white] (-4,0) -- (4,0);
\node[text=blue,xshift=0cm,yshift=4.25cm,fill=white,fill opacity=0.5]{~~~~~~~~~~~~~Put Cheezit inside the box~~~~~~~~~~~~~~~};
\node[text=blue,xshift=-2.0cm,yshift=1.75cm]{Start};
\node[text=blue,xshift=2.0cm,yshift=1.75cm]{Goal};
\node[text=blue,xshift=0cm,yshift=1.25cm,fill=white,fill opacity=0.5]{~~~~~~~~~~~~~Put Cheezit inside the  box~~~~~~~~~~~~~~};
\node[text=blue,xshift=-2.0cm,yshift=-1.25cm]{Start};
\node[text=blue,xshift=2.0cm,yshift=-1.25cm]{Goal};
\node[text=blue,xshift=0cm,yshift=-1.75cm,fill=white,fill opacity=0.5]{~~~~~Put Cheezit somewhere else on the table ~~~~~~};
\node[text=blue,xshift=-2.0cm,yshift=-4.25cm]{Start};
\node[text=blue,xshift=2.0cm,yshift=-4.25cm]{Goal};
\end{tikzpicture}
\caption{Pouring: Final solution varies according to the constraints}
\label{fig:pouring_3_examples}
\vspace{-2.0em}
\end{figure}


==> taskDefinitions.tex <==
We will analyze two tasks, which are defined as follows:

\begin{itemize}
\item{\textbf{Pick-and-place tasks:}  Given an object~\Object~in a start pose~\Tf{w}{s}~on
the table in front of the robot, the task
consists on repositioning it to a 3D goal position~\Pos{w}{g}~(not necessarily on the table). Both start and goal states must be
inside the reachable workspace of the robot arm being used. The task is considered successful if 
at the end of the pick-and-place task the object is set to~\Pos{w}{g}~with a small margin of error
to take into account arm control inaccuracies. Also, no collisions should happen during the execution.}
\item{\textbf{Pouring task:} Given a pouring object~\Object{P}~in a starting pose~\Tf{w}{s}~and a second container object~\Object{R}~, the goal of the task is to position~\Object{P}~over~\Object{R}~such that transfer of contents from~\Object{P}~to~\Object{R}~is feasible. In a geometrical context, pouring in this thesis is considered as a state
in which~\Object{P}~is placed above~\Object{R}~and its main principal axis form an angle $\in [0,-30]$ with the horizontal, such that~\Object{P}~is effectively pointing down.}
\end{itemize}

